A MegaCam Survey of Outer Halo Satellites. I. Description of the Survey

We describe a deep, systematic imaging study of satellites in the outer halo of the Milky Way. Our sample consists of 58 stellar overdensities --- i.e., substructures classified as either globular clusters, classical dwarf galaxies, or ultra-faint dwarf galaxies --- that are located at Galactocentric distances of R$_{\rm GC}$ > 25 kpc (outer halo) and out to ~400 kpc. This includes 44 objects for which we have acquired deep, wide-field, $g-$ and $r-$band imaging with the MegaCam mosaic cameras on the 3.6m Canada-France-Hawaii Telescope and the 6.5m Magellan-Clay telescope. These data are supplemented by archival imaging, or published $gr$ photometry, for an additional 14 objects, most of which were discovered recently in the Dark Energy Survey (DES). We describe the scientific motivation for our survey, including sample selection, observing strategy, data reduction pipeline, calibration procedures, and the depth and precision of the photometry. The typical 5$\sigma$ point-source limiting magnitudes for our MegaCam imaging --- which collectively covers an area of ~52 deg$^{2}$ --- are $g_{\rm lim}$ ~25.6 and $r_{\rm lim}$ ~25.3 AB mag. These limits are comparable to those from the coadded DES images and are roughly a half-magnitude deeper than will be reached in a single visit with LSST. Our photometric catalog thus provides the deepest and most uniform photometric database of Milky Way satellites available for the foreseeable future. In other papers in this series, we have used these data to explore the blue straggler populations in these objects, their density distributions, star formation histories, scaling relations and possible foreground structures.

==> hyperlink-year-only-natbib-patch.tex <==
% found on https://tex.stackexchange.com/questions/23227/how-to-hyperlink-only-the-year-part-when-using-natbib-and-hyperref

\RequirePackage{hyperref}
\RequirePackage{natbib}
\RequirePackage{etoolbox}

\makeatletter

% Patch case where name and year are separated by aysep
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

% Patch case where name and year are separated by opening bracket
\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\makeatother

